GENOME: GenerativE Neuro-symbOlic visual reasoning by growing and reusing ModulEs

Recent works have shown that Large Language Models (LLMs) could empower traditional neuro-symbolic models via programming capabilities to translate language into module descriptions, thus achieving strong visual reasoning results while maintaining the model's transparency and efficiency. However, these models usually exhaustively generate the entire code snippet given each new instance of a task, which is extremely ineffective. We propose generative neuro-symbolic visual reasoning by growing and reusing modules. Specifically, our model consists of three unique stages, module initialization, module generation, and module execution. First, given a vision-language task, we adopt LLMs to examine whether we could reuse and grow over established modules to handle this new task. If not, we initialize a new module needed by the task and specify the inputs and outputs of this new module. After that, the new module is created by querying LLMs to generate corresponding code snippets that match the requirements. In order to get a better sense of the new module's ability, we treat few-shot training examples as test cases to see if our new module could pass these cases. If yes, the new module is added to the module library for future reuse. Finally, we evaluate the performance of our model on the testing set by executing the parsed programs with the newly made visual modules to get the results. We find the proposed model possesses several advantages. First, it performs competitively on standard tasks like visual question answering and referring expression comprehension; Second, the modules learned from one task can be seamlessly transferred to new tasks; Last but not least, it is able to adapt to new visual reasoning tasks by observing a few training examples and reusing modules.

==> prompts/vqa_list.tex <==

%\begin{figure*}[b]
%\begin{lstlisting}[language=Python, xleftmargin=.15\textwidth,xrightmargin=.15\textwidth]
%\begin{lstlisting}[language=Python, xleftmargin=.1\textwidth,xrightmargin=.1\textwidth]
\begin{figure}
 \begin{minipage}[t]{\linewidth}
        %\centering
        \begin{minted}[
        frame=lines,
        framesep=2mm,
        fontsize=\footnotesize,
        bgcolor=Gray,
        numbersep=5pt,
        escapeinside=||,
        linenos
        ]{python}

Pre-defined Modules:
class LOC():
    """
    Generate boxes of the object on the image.
    Input:
        image: an image object
        object: an object string
    Output:
        box: a list of bounding boxes
	Examples:
	   BOX0=LOC(image=IMAGE,object='camel')
	"""
class COUNT():
    """
    Count the number of boxes in the list.
    Input:
        box: a list of bounding boxes
    Output:
        number: number of boxes
    Examples:
	ANSWER0=COUNT(box=BOX1)
    """
Suppose you are a program expert. Given a set of pre-defined modules, 
could you identify whether it is possible to write a program to get the
answer to the question? If not, what new modules do we need?
Note that you can only use the below pre-defined modules:
LOC, COUNT, CROP .......

Question: Is the purse to the left or to the right of the person?
Yes. The program is:
BOX0=LOC(image=IMAGE,object='person')
IMAGE0=CROP_LEFTOF(image=IMAGE,box=BOX0)
BOX1=LOC(image=IMAGE0,object='purse')
ANSWER0=COUNT(box=BOX1)
ANSWER1=EVAL(expr=f"'left' if {ANSWER0} > 0 else 'right'")
FINAL_RESULT=RESULT(var=ANSWER1)

Question: Which object is larger, the sphere or the blue cube?
No. We need to make a new module "COMPARE_SIZE" first. Here is the header
of the class:
class COMPARE_SIZE():
    """
    Compare the size of two objects in the image.
    One object is identified by the first bounding box of box0
    Another object is identified by the first bounding box of box1
    Input:
	image: an image object
        box0: a list of bounding boxes
        box1: a list of bounding boxes
    Output:
        flag: return True if first object is larger else False
    Examples:
	Question: Which object is larger, the sphere or the blue cube?
	BOX0=LOC(image=IMAGE,object='sphere')
	BOX1=LOC(image=IMAGE,object='blue cube')
	FLAG0=COMPARE_SIZE(image=IMAGE,box0=BOX0,box1=BOX1)
	ANSWER2=EVAL(expr=f"'sphere' if {FLAG0} else 'blue cube'")
	FINAL_RESULT=RESULT(var=ANSWER)
    """
.......
Question: __INSERT_NEW_QUESTION__
    \end{minted}
    \centering
\end{minipage}
    \vspace{-1.5em}
    \caption{Prompt of \ModuleA (Stage 1) to propose the module candidates.
    \label{prompt:stage1}
    }
\end{figure}


